Stochastic Policy Gradient Ascent in Reproducing Kernel Hilbert Spaces

Reinforcement learning consists of finding policies that maximize an expected cumulative long-term reward in a Markov decision process with unknown transition probabilities and instantaneous rewards. In this paper, we consider the problem of finding such optimal policies while assuming they are continuous functions belonging to a reproducing kernel Hilbert space (RKHS). To learn the optimal policy we introduce a stochastic policy gradient ascent algorithm with three unique novel features: (i) The stochastic estimates of policy gradients are unbiased. (ii) The variance of stochastic gradients is reduced by drawing on ideas from numerical differentiation. (iii) Policy complexity is controlled using sparse RKHS representations. Novel feature (i) is instrumental in proving convergence to a stationary point of the expected cumulative reward. Novel feature (ii) facilitates reasonable convergence times. Novel feature (iii) is a necessity in practical implementations which we show can be done in a way that does not eliminate convergence guarantees. Numerical examples in standard problems illustrate successful learning of policies with low complexity representations which are close to stationary points of the expected cumulative reward.

==> convergence_pars_bkp.tex <==
%!TEX root = root.tex

\section{Convergence Analysis of Sparse Policy Gradient}\label{sec_convergence_pars}


This section contains the proof of Theorem \ref{theo_parsimonious}. It starts by providing a lower bound on the expectation of random variables $U(h_{k+1})$ conditioned to the sigma field $\ccalF_k$ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% L E M M A     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{lemma}\label{lemma_supermartingale_pars}
  %
  The sequence of random variables $U(h_k)$ satisfies the following inequality 
  %
\begin{equation}\label{eqn_supermartingale_equation_pars}
    \begin{split}
      \mathbb{E}\left[{U(h_{k+1})|\ccalF_k}\right] &\geq  U(h_k)- \eta^2 C\\
      &\hspace{-1cm}+\eta\left\|\nabla_h U(h_k)\right\|_\ccalH\left(\left\|\nabla_h U(h_k)\right\|_\ccalH -\frac{\epsilon}{\eta}\right), 
\end{split}
\end{equation}
%
where $C$ is the following positive constant
%
\begin{equation}\label{eqn_bound_for_radius_convergence}
C = L_1\left(\sigma^2+2\frac{\epsilon}{\eta}\sigma +\frac{\epsilon^2}{\eta^2}\right)+\eta L_2\left(\sigma^2+2\frac{\epsilon}{\eta}\sigma +\frac{\epsilon^2}{\eta^2}\right)^{3/2},
\end{equation}
%
where  $L_1$ and $L_2$ are the constants defined in Lemma \ref{lemma_lipchitz} and $\sigma$ is the constant defined in 
Lemma \ref{lemma_stochastic_gradient}.
  \end{lemma}
\begin{proof}
  Consider the Taylor expansion of $U(h_{k+1})$ around $h_k$,
  %
  \begin{equation}
    \begin{split}
       U(h_{k+1})= U(h_k)+\left<\nabla_h U(f_k,\cdot),h_{k+1}-h_k\right>_{\ccalH}.\label{Taylor}
      \end{split}
  \end{equation}
  %
 where $f_k = \lambda h_k +(1-\lambda)h_{k+1}$ with $\lambda\in[0,1]$. Adding and subtracting $\left<\nabla_h U(h_k,\cdot),h_{k+1}-h_k\right>_{\ccalH}$ to the previous expression, using the Cauchy-Schwartz inequality and the result of Lemma \ref{lemma_lipchitz} we can rewrite \eqref{Taylor} as 
  \begin{equation}
    \begin{split}
     U(h_{k+1}) 
     &= U(h_k)+\left<\nabla_h U(h_k,\cdot),h_{k+1}-h_k\right>_{\ccalH} \\
     &+\left<\nabla_h U(f_k,\cdot)-\nabla_hU(h_k,\cdot),h_{k+1}-h_k\right>_{\ccalH}\\
     %&\geq U(h_k)+\left<\nabla_h U(h_k,\cdot),h_{k+1}-h_k\right>_{\ccalH} \\
     %&-\left\|\nabla_h U(f_k,\cdot)-\nabla_hU(h_k,\cdot)\right\|_\ccalH\left\|h_{k+1}-h_k\right\|_{\ccalH}\\
     & \geq U(h_k)+\left<\nabla_h U(h_k,\cdot),h_{k+1}-h_k\right>_{\ccalH} \\
     &-L_1\left\|h_{k+1}-h_k\right\|_{\ccalH}^2-L_2\left\|h_{k+1}-h_k\right\|_{\ccalH}^3.
      \end{split}
  \end{equation}
  %
  Let us consider the conditional expectation of the random variable $U(h_{k+1})$ with respect to the sigma-field $\ccalF_k$. Combine the monotonicity and the linearity of the expectation with the fact that $h_k$ is measurable with respect to $\ccalF_k$ to write
  %
  \begin{align}\nonumber
          &\mathbb{E}\left[{U(h_{k+1})|\ccalF_k}\right] \geq U(h_k)+\left<\nabla_h U(h_k,\cdot),\mathbb{E}\left[h_{k+1}-h_k|\ccalF_k\right]\right>_{\ccalH} \\
      &\hspace{-.1cm}-\hspace{-.1cm}L_1\mathbb{E}\hspace{-.1cm}\left[\left\|h_{k+1}-h_k\right\|_{\ccalH}^2|\ccalF_k\right]\hspace{-.1cm}-\hspace{-.1cm}L_2\mathbb{E}\hspace{-.1cm}\left[\left\|h_{k+1}-h_k\right\|_{\ccalH}^3|\ccalF_k\right]\hspace{-.1cm}.
     \label{eqn_first_supermartingale_bound_pars}
    \end{align}
  %
  Substitute \eqref{bias_bk} for $h_{k+1}$  to write the expectation of the quadratic term in the right hand side of \eqref{eqn_first_supermartingale_bound_pars} as 
  %
  \begin{align*}
         L_1\mathbb{E}&\left[\left\|h_{k+1}-h_k\right\|_{\ccalH}^2|\ccalF_k\right] = L_1\mathbb{E}\left[\left\|\eta \hat{\nabla}_h U(h,\cdot)+b_k\right\|_{\ccalH}^2|\ccalF_k\right] \\
     \leq  L_1&\left(\eta^2 \mathbb{E}\left[\left\|\hat{\nabla}_h U(h_k,\cdot)\right\|_{\ccalH}^2|\ccalF_k\right]\right.\\
		&\left.+2\eta\epsilon\mathbb{E}\left[\left\|\hat{\nabla}_h U(h_k,\cdot)\right\|_{\ccalH}|\ccalF_k\right]+\epsilon^2 \right),
 \end{align*}
  
  where we have used that $\|b_k\|\leq \epsilon$ as stated in Proposition \ref{prop_error_bound}. Using the bounds provided in  Lemma \ref{lemma_stochastic_gradient}, the previous expression can be upper bounded by
  %
  \begin{equation}\label{eleuno}
    L_1\mathbb{E}\left[\left\|h_{k+1}-h_k\right\|_{\ccalH}^2|\ccalF_k\right] \leq \eta^2L_1\left(\sigma^2+2\frac{\epsilon}{\eta}\sigma +\frac{\epsilon^2}{\eta^2}\right).
    \end{equation}
  %
  With a similar procedure we obtain
  \begin{equation}\label{eledos}
    \begin{split}
      L_2\mathbb{E}\left[\left\|h_{k+1}-h_k\right\|_{\ccalH}^3|\ccalF_k\right] \leq \eta^2 \eta_0L_2\left(\sigma^2+2\frac{\epsilon}{\eta}\sigma +\frac{\epsilon^2}{\eta^2}\right)^{3/2}
      \end{split}
    \end{equation}
  %
  Observe that the sum of \eqref{eleuno} and \eqref{eledos} is equal to $\eta^2C$ in \eqref{eqn_bound_for_radius_convergence}. Then, substitute \eqref{eleuno} and \eqref{eledos} in  \eqref{eqn_first_supermartingale_bound_pars} to obtain
  %  
  \begin{equation}
    \begin{split}\label{eqn_martigale_innerproduct}
      \mathbb{E}\left[{U(h_{k+1})|\ccalF_k}\right] &\geq U(h_k)-C\eta^2\\
&      +\left<\nabla_h U(h_k),\mathbb{E}\left[h_{k+1}-h_k|\ccalF_k\right]\right>_{\ccalH}. 
\end{split}
    \end{equation}
  %
  Finally, \eqref{eqn_supermartingale_equation_pars} results from applying the Cauchy-Schwartz inequality   to the inner product in \eqref{eqn_martigale_innerproduct} and then substituting \eqref{bias_bk} for $h_{k+1}$, with $\|b_k\|\leq \epsilon$. 

%  we can write the inner product on the previous equation as
  %
%  \begin{equation}
%\left<\nabla_h U(h_k),\mathbb{E}\left[h_{k+1}-h_k|\ccalF_k\right]\right>_{\ccalH} = \eta\%left\|\nabla_h U(h_k)\right\|^2_{\ccalH}+\left<\nabla_h U(h_k), b_k\right>_{\ccalH}.
%    \end{equation}
  %
%The proof is then completed using the Cauchy-Schwartz inequality and fact that the norm of the bias is bounded by $\epsilon$ (cf., Proposition \ref{prop_error_bound}).
  %
  \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% M A I N              M A T T E R %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The previous Lemma establishes a lower bound on the expectation of $U(h_{k+1})$ conditioned to the sigma algebra $\ccalF_k$. This lower bound however, is not enough for $U(h_k)$ to be a submartingale, since the sign of the term added to $U(h_k)$ in the right hand side of \eqref{eqn_supermartingale_equation_pars} depends on the norm of $\nabla_h U(h_k)$. This is in contrast with the situation in Lemma \ref{lemma_supermartingale}, where the term was always positive. The origin of this issue lies on the bias introduced by the sparsification. However, when the norm of the gradient is large the term is negative and we have a submartingale while a neighborhood of the critical point is not reached. To formalize this idea let us define the neighborhood as
 %
 \begin{equation}\label{neigborhood_inequality}
\left\|\nabla_h U(h_k,\cdot)\right\|_{\ccalH} \leq \frac{\epsilon}{2\eta}+\frac{\sqrt{\epsilon^2+4\eta^3C}}{2\eta},
\end{equation}
 and the corresponding stopping time
%This idea will be formalized in the following lemma to establish that the limit inferior of the norm of the gradient is bounded by a quantity that can be made arbitrarily small. This means, that the iterates visit the neighborhood of the critical point infinitely often. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% L E M M A %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{lemma}
%  Let $\eta = \eta>0$ and $\epsilon_k = \varepsilon$ for all $k\geq 0$. Then with probability one we have that
  %
%  \begin{equation}\label{eqn_liminf}
%    \liminf_{k\to\infty} \left\|\nabla_h U(h_k,\cdot)\right\|_{\ccalH} \leq \frac{\vareps%ilon}{2\eta}+\frac{\sqrt{\varepsilon^2+4\eta^3B}}{2\eta}.
%    \end{equation}
  %
%\end{lemma}
%\begin{proof}
  %
%  Let us define the following stopping time
  %
  \begin{equation}
N = \min_{k\geq 0} \left\{\left\|\nabla_h U(h_{k},\cdot)\right\|_{\ccalH} \leq \frac{\epsilon}{2\eta}+\frac{\sqrt{\epsilon^2+4\eta^3C}}{2\eta}  \right\}.
    \end{equation}
  
	In order to prove  \eqref{eqn_liminf} we will argue that either the limit exists and satisfies the bound in \eqref{eqn_liminf}, or $P(N<\infty)=1$, in which case \eqref{neigborhood_inequality} must be recursively satisfied after a finite number of iterations so that  \eqref{eqn_liminf} holds.  
  In this direction we define $V_k=\left(U(h^*)-U(h_{k})\right)\mathbbm{1}(k-1\leq N)$, with $\mathbbm{1}(\cdot)$ being the indicator function, and prove that $V_k$ is a non-negative submartingale. Indeed, since $U(h^*)$ maximizes $U(h)$, $V_k$ is always non-negative. In addition $V_k\in \ccalF_k$ since $U(h_k)\in\ccalF_k$ and $\mathbbm{1}(k-1\leq N)\in\ccalF_{k-1}\subset \ccalF_{k}$. To show that $\mathbb{E}[V_{k+1} | \ccalF_k] \leq V_k$ start by using that $\mathbbm{1}(k\leq N)\in\ccalF_{k}$ and write
  %
  \begin{equation}
\mathbb{E}\left[V_{k+1} | \ccalF_k\right]  =  \mathbbm{1}(k\leq N) \mathbb{E}\left[U(h^*)-U(h_{k+1}) | \ccalF_k\right] 
    \end{equation}
  %
  Using \eqref{eqn_supermartingale_equation_pars} we can upper bound $\mathbb{E}\left[V_{k+1} | \ccalF_k\right]$ as
  %
  \begin{align}\label{eqn_supermartingale_equation_pars_stop}
  &\mathbb{E}\left[V_{k+1} | \ccalF_k\right]  \leq  \mathbbm{1}(k\leq N)  \left(U(h^*)-\hspace{-.1cm}U(h_{k})\right)- \mathbbm{1}(k \leq N)W_k.
\end{align}
  %
	with
  \begin{align}
W_k &:= \eta \left\|\nabla_hU(h_k,\cdot) \right\|_{\ccalH}^2 - \epsilon \left\|\nabla_hU(h_k,\cdot) \right\|_{\ccalH} - \eta^2 C   \label{eqn_def_wk}
  \end{align}
	
Notice that the bound in \eqref{neigborhood_inequality} is root of \eqref{eqn_def_wk} as a polynomial in the variable $\left\|\nabla_hU(h_k,\cdot) \right\|$. It follows that   $W_k>0$ as long as $k< N$. Also notice that the indicator function $\mathbbm{1}(k\leq N)$ is non-increasing with $k$. Using these two facts together  it follows from \eqref{eqn_supermartingale_equation_pars_stop} that $\mathbb{E}[V_{k+1} | \ccalF_k] \leq V_k$. Thus, $V_k$ is a nonnegative submartingale and therefore it converges to random variable $V$ such that $\mathbb{E}[V]\leq \mathbb{E}[V_0]$ (see e.g., \cite[Theorem 5.29]{durrett2010probability}).
%
Rearranging the terms in \eqref{eqn_supermartingale_equation_pars_stop} and considering the total expectation in both sides of the inequality we have that 
  %
\begin{equation}\label{eqn_supermartingale_equation_pars_before_limit}
  \begin{split}
   \mathbb{E}\left[\sum_{j = 0}^{k}W_k  \right]    \leq \mathbb{E}[V_0] -\mathbb{E}\left[ V_{k+1} \right] .
   \end{split}
    \end{equation}
 %
 By definition of the stopping time $N$, $W_k$ is nonnegative, and thus the sequence of random variables
 %
 \begin{equation}
S_k = \sum_{j = 0}^{k}\mathbbm{1}(j \leq N)W_j,
 \end{equation}
 %
 is monotonically increasing. Hence, use the Monotone Convergence Theorem (see e.g.,\cite[Theorem 1.6.6]{durrett2010probability}) to write 
 %
 \begin{equation}\label{eqn_supermartingale_equation_pars_limit1}
   \begin{split}
     \lim_{k\to\infty} \mathbb{E}\left[\sum_{j = 0}^{k}\mathbbm{1}(j \leq N)W_j \right] =\mathbb{E}\left[\sum_{j = 0}^{\infty}\mathbbm{1}(j \leq N)W_j  \right].
\end{split}.
   \end{equation}
On the other hand, because $V_K$ is a bounded sequence by virtue of the Dominated Convergence Theorem (see e.g. \cite[Theorem 1.6.7]{durrett2010probability}) we have that 
  %
  \begin{equation}\label{eqn_supermartingale_equation_pars_limit2}
\mathbb{E}[V] = \mathbb{E}[\lim_{k\to\infty} V_k] = \lim_{k\to \infty} \mathbb{E}[V_k].
    \end{equation}
  %
  Taking the limit of $k$ going to infinity in both sides of \eqref{eqn_supermartingale_equation_pars_before_limit} and using \eqref{eqn_supermartingale_equation_pars_limit1} and \eqref{eqn_supermartingale_equation_pars_limit2} we have that 
  %
  \begin{equation}\begin{split}
    \mathbb{E}\left[\sum_{j = 0}^{\infty}\mathbbm{1}(j \leq N)W_j  \right] \leq \mathbb{E}[V_0]-\mathbb{E}[V] < \infty.
    \end{split}
    \end{equation}
  %
  Observe that the expectation on the left hand side of the previous expression can be computed as
  %
  \begin{equation}
    \begin{split}
%      \mathbb{E}\left[\sum_{j = 0}^{\infty}\mathbbm{1}(j \leq N)\left(\eta\left\|\nabla_h U(h_{j},\cdot)\right\|^2\right.\right.\\
 %       \left.\left.-\left\| \nabla_h U(h_{j},\cdot)\right\|\epsilon-\eta^2 B\right)  \right] \\
      %=
      P(N<\infty)      \mathbb{E}\left[\sum_{j = 0}^{N}W_j  \Big| N<\infty \right] 
      + P(N=\infty)      \mathbb{E}\left[\sum_{j = 0}^{\infty}W_j \Big| N=\infty \right]. 
\end{split}
    \end{equation}
  %
 By virtue of Lemma \ref{lemma_bounded_gradient}, $\left\| \nabla_h U(h,\cdot) \right\|$ is bounded for all $h\in\ccalH$. Thus the first sum in the right hand side of the previous expression is bounded. Therefore it holds that 
  %
  \begin{equation} 
P(N=\infty)      \mathbb{E}\left[\sum_{j = 0}^{\infty}W_j\Big| N=\infty  \right]  <\infty.
%
  \end{equation}
  %
  The latter can only hold if $P(N=\infty) = 0$ or if the expectation of the sum is bounded. If the former happens it means that infinitely often we revisit the neighborhood satisfying \eqref{neigborhood_inequality}
  %
  and thus the sequence satisfies \eqref{eqn_liminf}. It remains to analyze the case where the sum of the expectation is bounded. Using the Monotone Convergence Theorem one can exchange the sum with the expectation and therefore we have that
  %
  \begin{equation}
\sum_{j = 0}^{\infty}    \mathbb{E}\left[W_j\Big| N=\infty  \right]  <\infty,
  \end{equation}
  %
  which implies that $\lim_{k\to\infty} \mathbb{E}[W_k|N=\infty] =0$. Thus 
  %
  \begin{equation}
    \lim_{k\to\infty}\mathbb{E}\left[\left(\eta\left\|\nabla_h U(h_{k},\cdot)\right\|^2-\left\| \nabla_h U(h_{k},\cdot)\right\|\epsilon-\eta^2 C\right)\right] = 0.
    \end{equation}
  %
  Moreover, because the norm of the gradient is bounded, the Dominated Convergence Theorem allows us to write
  %
    \begin{equation}
    \mathbb{E}\left[\lim_{k\to\infty}\left(\eta\left\|\nabla_h U(h_{k},\cdot)\right\|^2-\left\| \nabla_h U(h_{k},\cdot)\right\|\epsilon-\eta^2 C\right)\right] = 0.
    \end{equation}
    %
    Because the random variable is nonnegative it must hold that 
  \begin{equation}
\lim_{k\to\infty} \left\|\nabla_h U(h_k,\cdot)\right\|_{\ccalH} = \frac{\epsilon}{2\eta}+\frac{\sqrt{\epsilon^2+4\eta^3C}}{2\eta}.
    \end{equation}
  %
  Thus, \eqref{eqn_liminf} holds as well if $P(N=\infty)>0$. It remains to be shown that the model order of the representation is bounded for all $k$. The proof of this result is identical to that in \cite[Theorem 3]{koppel2016parsimonious}.
%\end{proof}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% P R O P O S I T I O N  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{proposition}
%Let $M_k$ be the model order of $h_k$, i.e., the number of columns of the dictionary $\bbD_k$ which parametrizes $h_k$. Then, there exists a finite upper bound $M^\infty$ such that, for all $k\geq 0$, the model order is always bounded as $M_k\leq M^\infty$. 
%  \end{proposition}
%\begin{proof}
%The proof is the same as that of \cite[Theorem 3]{koppel2016parsimonious}.
%  \end{proof}


==> introduction.tex <==
%!TEX root = root.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   A   B   S   T   R   A   C   T   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{abstract}
  In this work we consider the problem of policy optimization in the context of reinforcement learning. In order to avoid discretization, we select the optimal policy to be a continuous function belonging to a reproducing Kernel Hilbert Space (RKHS) which maximizes a expected  cumulative reward (ECR). We design a policy gradient  algorithm (PGA) in this context, deriving the gradients of the functional ECR and  learning the unknown state transition probabilities on the way. In particular, we propose an unbiased stochastic approximation for the gradient that requires a finite number of steps. This unbiased estimator is the key enabler for a novel stochastic PGA, which provably converges to a critical point of the ECR. However, the RKHS approach increases the model order per iteration by adding extra kernels, which may render the numerical complexity prohibitive. To overcome this limitation, we prune the kernel dictionary using an orthogonal matching pursuit procedure, and  prove that the modified method keeps the model order bounded for all iterations, while ensuring convergence to a neighborhood of the critical point.
\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Introduction}
Reinforcement learning is a model-free control technique that consists of learning the best action that can be performed given a current state through rewards given to the agent depending on the quality of the actions selected \cite{sutton1998reinforcement}. This framework is specially suited to address sequential decision making under uncertainty and have gained broad interest in robotics \cite{kober2013reinforcement}, control \cite{shreve1978alternative} and finance \cite{rasonyi2005utility}.

The objective in the previous framework is to select actions that maximize the expected value of the cumulative rewards. One of the most celebrated algorithms in reinforcement learning is q-learning \cite{watkins1992q} where the objective is to learn the q-function that describes the cumulative rewards. Then, once the system reaches a given state, the next action is selected to maximize the learned q-function. This is a drawback of q-learning since the q-function is typically non-convex so that finding the action that maximizes it is not always an easy task. A more direct approach is pursued by the class of policy gradient  where one aims to learn the optimal map from states to actions directly \cite{sutton2000policy,deisenroth2013survey}.

Another drawback of classic reinforcement learning algorithms is that they suffer from the curse of dimensionality that results from discretization \cite{friedman2001elements}. This is, the complexity of the problem increases combinatorially with the number of states and actions that are needed to represent the state-action space with sufficient precision. This is not surprising since from an optimization standpoint it is known that discretizing a continuous space may render a convex problem   NP-Hard. Efforts in providing versions of these algorithms for continuous state spaces have been pursued. In \cite{koppel2017breaking,tolstayanonparametric} the aim is to represent the expected cumulative reward as a continuous function of the state and the actions. To do so, it is assumed that such function belongs to a Reproducing Kernel Hilbert Space (RKHS). Likewise, RKHS-based policy gradient methods have been considered, where the optimal mapping from states to actions is a continuous function \cite{lever2015modelling}.  

In this work, we consider policy learning in RKHS as in \cite{lever2015modelling}. Our main contribution is related to the construction of the estimate of the gradient of the expected cumulative reward (Section \ref{sec_algorithm}). In particular, we provide an algorithm to obtain an unbiased estimate of such gradient in a finite number of steps. On the way, we gain intuition on the use of  random Gaussian policies, showing that they provide tractable versions of the q-function gradient, and that by stochastic approximation  they achieve numerical differentiation. We also establish convergence of the gradient ascent algorithm in the RKHS. The previous algorithm however, suffers from memory explosion. To overcome this limitation we use orthogonal match and pursuit \cite{vincent2002kernel} to control the order of the model required to represent the policy (Section \ref{sec_komp}). Other than concluding remarks the paper ends with numerical experiments (Section \ref{sec_numerical}) where we consider the mountain car problem (Section \ref{sec_mountain_car}) and a navigation problem in a space with obstacles (Section \ref{sec_sim_online}).





==> proof_of_proposition_zero.tex <==
%!TEX root = root.tex

\section{Policy gradient proof}

To compute policy gradients, we recall the definition of the Value function
%
\begin{align}\label{eqn_pf_zero_value_function}
  V(s_0; \pi) :=& \mbE \bigg [\sum_{t=0}^\infty  r(s_t, a_t) \given s_0\bigg] \nonumber \\
             =& \int \sum_{t=0}^\infty  r(s_t, a_t) \, p( s_{1:\infty}, a_{0:\infty} \given s_0) ,
\end{align}
%
as well as the definition of the Q-function
%
\begin{align}\label{eqn_pf_zero_q_function}
  Q(s_0, a_0; \pi) 
    :=& \mbE \bigg [\sum_{t=0}^\infty  r(s_t, a_t) \given s_0, a_0 \bigg] \nonumber \\
     =& \int \sum_{t=0}^\infty  r(s_t, a_t) \, p (s_{1:\infty}, a_{1:\infty} \given s_0, a_0) ,
\end{align}
%
Given the expressions in \eqref{eqn_pf_zero_value_function} and \eqref{eqn_pf_zero_q_function}, it follows that the Q-function and the value function differ on the marginalization with respect to the action which is present in the value function but is not present in the Q-function. Since that marginal distribution is, by definition, the policy $\pi(a_0\given s_0)$ we can write
%
\begin{align}\label{eqn_pf_zero_value_function_in_terms_of_q_function}
  V(s_0; \pi) = \int Q(s_0, a_0; \pi) \pi(a_0 \given s_0) .
\end{align}
%
It is also possible to write the Q-function in terms of the value function. This requires letting the system run for one iteration, which yields
%
\begin{align}\label{eqn_pf_zero_q_function_in_terms_of_value_function}
   Q(s_0, a_0; \pi) = r (s_0,a_0) + \gamma \int V(s_1; \pi) \, p(s_1\given s_0, a_0) .
\end{align}
%
Policy gradients can be evaluated from \eqref{eqn_pf_zero_value_function_in_terms_of_q_function} which, due to linearity of expectation and integral operators, yields 
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient}
  \nabla_\pi V(s_0; \pi) 
     = &\int            Q(s_0, a_0; \pi) \nabla_\pi \pi(a_0 \given s_0) + \nonumber\\
       &\int \nabla_\pi Q(s_0, a_0; \pi)            \pi(a_0 \given s_0) .
\end{align}
%
In the first summand of \eqref{eqn_pf_zero_policy_value_function_gradient} we have $\nabla_\pi \pi(a_0 \given s_0)$. This results in an interesting expression where $Q(s_0, a_0; \pi)$ is integrated uniformly with respect to all actions. To clarify that the integral is with respect to $a_0$ given $a_0$ we write 
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_summand_one}
   \int Q(s_0, a_0; \pi) \nabla_\pi \pi(a_0 \given s_0) 
        = \int Q(s_0, a_0; \pi)\, d (a_0 \given s_0).
\end{align}
%
For the second summand of \eqref{eqn_pf_zero_policy_value_function_gradient} we use \eqref{eqn_pf_zero_q_function_in_terms_of_value_function} to evaluate $\nabla_\pi Q(s_0, a_0; \pi)$. In computing this, we observe that the collected reward $r (s_0,a_0)$ when given $s_0$ and $a_0$ does not depend on the policy and that neither does the transition probability $p(s_1\given s_0, a_0)$. Therefore, the gradient of the Q-function with respect to the policy $\pi$ can be written as 
%
\begin{align}\label{eqn_pf_zero_q_function_gradient}
   \nabla_\pi Q(s_0, a_0; \pi) = \gamma \int \nabla_\pi V(s_1; \pi) p(s_1\given s_0, a_0) .
\end{align}
%
Substituting \eqref{eqn_pf_zero_q_function_gradient} and \eqref{eqn_pf_zero_policy_value_function_gradient_summand_one} into \eqref{eqn_pf_zero_policy_value_function_gradient} yields 
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_two}
  \nabla_\pi V(s_0; \pi) 
     = &\int Q(s_0, a_0; \pi)\, d (a_0 \given s_0) + \nonumber\\
       &\gamma \int \nabla_\pi V(s_1; \pi) p(s_1\given s_0, a_0) \pi(a_0 \given s_0) .
\end{align}
%
We further observe that the marginalization $p(s_1\given s_0, a_0) \pi(a_0 \given s_0)$ results in evaluating the distribution $p(s_1\given s_0)$ from where \eqref{eqn_pf_zero_policy_value_function_gradient_two} reduces to
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_three}
  \nabla_\pi V(s_0; \pi) 
     = &\int Q(s_0, a_0; \pi)\, d (a_0 \given s_0) + \nonumber\\
       &\gamma \int \nabla_\pi V(s_1; \pi) p(s_1\given s_0) .
\end{align}
%
We now need to evaluate the gradient $\nabla_\pi V(s_1; \pi)$ but doing this simply requires repeating the steps in \eqref{eqn_pf_zero_policy_value_function_gradient} - \eqref{eqn_pf_zero_policy_value_function_gradient_three}. When doing this we obtain
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_recursion}
  \nabla_\pi V(s_0; \pi) 
     = &\int Q(s_0, a_0; \pi)\, d (a_0 \given s_0) + \nonumber\\
       &\gamma   \int Q(s_1, a_1; \pi)\, d (a_1 \given s_1) p(s_1\given s_0)  + \nonumber\\ 
       &\gamma^2 \int \nabla_\pi V(s_1; \pi) p(s_2\given s_0) p(s_1\given s_0) .
\end{align}
%
If we keep repeating this procedure we obtain
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_recursion_complete}
  \nabla_\pi V(s_0; \pi) 
     = &\sum_{t=0}^{\infty} \gamma^t\int Q(s_t, a_t; \pi)\, d (a_t \given s_t) p(s_t\given s_0) .
\end{align}
%
Defining the probability distribution of ever visiting $s_t$ yields
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_recursion_complete}
  \nabla_\pi V(s_0; \pi) 
     = & \int Q(s_t, a_t; \pi)\, d (a_t \given s_t) \rho(s_t\given s_0) .
\end{align}
%
And using the log trick for the policy $\pi(a_t\given s_t)$
%
\begin{align}\label{eqn_pf_zero_policy_value_function_gradient_recursion_complete}
  \nabla_\pi V(s_0; \pi) 
     = & \int Q(s_t, a_t; \pi) \nabla_\pi \log(\pi(a_t\given s_t))\, \rho(a_t, s_t\given s_0) .
\end{align}
%






